Alpha-constrained QSE Nucleosynthesis in High-entropy and Fast-expanding Material

We investigate the nucleosynthesis process in high-entropy ($s/k_{\rm B}\gtrsim100$) and very fast-expanding ($\tau_{\rm exp}\sim10^{-3}\ {\rm s}$) materials. In such a material with the electron fraction near 0.5, an interesting nucleosynthesis process occurs. In this process, the abundance distribution of heavy-nuclei of $A>100$ achieve quasi-statistical equilibrium (QSE) at high temperature and the abundances are frozen at the end of the nucleosynthesis. We explain this abundance distribution using the "alpha-constrained QSE" abundances formulated in this paper. We demonstrate that this nucleosynthesis would occur in neutrino-driven winds from massive proto-neutron stars in hypernovae, where $A\sim140$ $p$-nuclei are synthesized.

==> bib.tex <==
\bibliographystyle{apj}
\begin{thebibliography}{108}
\expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi

\bibitem[Anders 
\& Grevesse(1989)]{1989GeCoA..53..197A} Anders, E., \& Grevesse, N.\ 1989, \gca, 53, 197 

\bibitem[Cardall 
\& Fuller(1997)]{1997ApJ...486L.111C} Cardall, C.~Y., \& Fuller, G.~M.\ 1997, \apjl, 486, L111

\bibitem[Cooperstein et al.(1986)]{1986ApJ...309..653C} Cooperstein, J., 
van den Horn, L.~J., \& Baron, E.~A.\ 1986, \apj, 309, 653

\bibitem[Cyburt et al.(2010)]{2010ApJS..189..240C} Cyburt, R.~H., Amthor, 
A.~M., Ferguson, R., et al.\ 2010, \apjs, 189, 240 

\bibitem[Freiburghaus et al.(1999)]{1999ApJ...525L.121F} Freiburghaus, C., 
Rosswog, S., \& Thielemann, F.-K.\ 1999, \apjl, 525, L121

\bibitem[Fuller et al.(1985)]{1985ApJ...293....1F} Fuller, G.~M., Fowler, 
W.~A., \& Newman, M.~J.\ 1985, \apj, 293, 1

\bibitem[Graboske et al.(1973)]{1973ApJ...181..457G} Graboske, H.~C., 
Dewitt, H.~E., Grossman, A.~S., \& Cooper, M.~S.\ 1973, \apj, 181, 457 

\bibitem[Hoffman et al.(1997)]{1997ApJ...482..951H} Hoffman, R.~D., 
Woosley, S.~E., \& Qian, Y.-Z.\ 1997, \apj, 482, 951

\bibitem[Honda et al.(2006)]{2006ApJ...643.1180H} Honda, S., Aoki, W., 
Ishimaru, Y., Wanajo, S., \& Ryan, S.~G.\ 2006, \apj, 643, 1180

\bibitem[Horiguchi et al.(1996)]{Horiguchi+(1996)} Horiguchi, T., Tachibana,T., \& Katakura, J.,  Japanese Nuclear Data Committee (JNDC) and JAERI Nuclear Data Center,1996

\bibitem[Itoh et al.(1979)]{1979ApJ...234.1079I} Itoh, N., Totsuji, H., 
Ichimaru, S., \& Dewitt, H.~E.\ 1979, \apj, 234, 1079 

\bibitem[Iwamoto et al.(1998)]{1998Natur.395..672I} Iwamoto, K., Mazzali, 
P.~A., Nomoto, K., et al.\ 1998, \nat, 395, 672

\bibitem[Iwamoto et al.(2000)]{2000ApJ...534..660I} Iwamoto, K., Nakamura, 
T., Nomoto, K., et al.\ 2000, \apj, 534, 660

\bibitem[Langanke 
\& Mart{\'{\i}}nez-Pinedo(2001)]{2001ADNDT..79....1L} Langanke, K., \& Mart{\'{\i}}nez-Pinedo, G.\ 2001, Atomic Data and Nuclear Data Tables, 79, 1

\bibitem[Mazzali et al.(2002)]{2002ApJ...572L..61M} Mazzali, P.~A., Deng, 
J., Maeda, K., et al.\ 2002, \apjl, 572, L61 

\bibitem[Mazzali et al.(2003)]{2003ApJ...599L..95M} Mazzali, P.~A., Deng, 
J., Tominaga, N., et al.\ 2003, \apjl, 599, L95 

\bibitem[M{\"o}ller et al.(2003)]{2003PhRvC..67e5802M} M{\"o}ller, P., 
Pfeiffer, B., \& Kratz, K.-L.\ 2003, \prc, 67, 055802 

\bibitem[Oda et al.(1994)]{1994ADNDT..56..231O} Oda, T., Hino, M., Muto, 
K., Takahara, M., 
\& Sato, K.\ 1994, Atomic Data and Nuclear Data Tables, 56, 231 

\bibitem[Otsuki et al.(2000)]{2000ApJ...533..424O} Otsuki, K., Tagoshi, H., 
Kajino, T., \& Wanajo, S.-y.\ 2000, \apj, 533, 424

\bibitem[Pruet et al.(2006)]{2006ApJ...644.1028P} Pruet, J., Hoffman, 
R.~D., Woosley, S.~E., Janka, H.-T., \& Buras, R.\ 2006, \apj, 644, 1028

\bibitem[Qian \& Woosley(1996)]{1996ApJ...471..331Q} Qian, Y.-Z., \& Woosley, S.~E.\ 1996, \apj, 471, 331

\bibitem[Rauscher et al.(2002)]{2002ApJ...576..323R} Rauscher, T., Heger, 
A., Hoffman, R.~D., \& Woosley, S.~E.\ 2002, \apj, 576, 323

\bibitem[Rayet et 
al.(1995)]{1995A&A...298..517R} Rayet, M., Arnould, M., Hashimoto, M., Prantzos, N., \& Nomoto, K.\ 1995, \aap, 298, 517 

\bibitem[Roberts et al.(2010)]{2010ApJ...722..954R} Roberts, L.~F., 
Woosley, S.~E., \& Hoffman, R.~D.\ 2010, \apj, 722, 954

\bibitem[Sekiguchi et al.(2012)]{2012PTEP.2012aA304S} Sekiguchi, Y., 
Kiuchi, K., Kyutoku, K., 
\& Shibata, M.\ 2012, Progress of Theoretical and Experimental Physics, 2012, 010000 

\bibitem[Tachibana(2000)]{Tachibana(2000)} Tachibana, T., private communication

\bibitem[Takahashi 
\& Yokoi(1987)]{1987ADNDT..36..375T} Takahashi, K., \& Yokoi, K.\ 1987, Atomic Data and Nuclear Data Tables, 36, 375 

\bibitem[Thompson et al.(2001)]{2001ApJ...562..887T} Thompson, T.~A., 
Burrows, A., \& Meyer, B.~S.\ 2001, \apj, 562, 887

\bibitem[Timmes 
\& Swesty(2000)]{2000ApJS..126..501T} Timmes, F.~X., \& Swesty, F.~D.\ 2000, \apjs, 126, 501

\bibitem[Wanajo et al.(2001)]{2001ApJ...554..578W} Wanajo, S., Kajino, T., 
Mathews, G.~J., \& Otsuki, K.\ 2001, \apj, 554, 578

\bibitem[Wanajo(2006)]{2006ApJ...647.1323W} Wanajo, S.\ 2006, \apj, 647, 
1323

\bibitem[Wanajo et al.(2014)]{2014ApJ...789L..39W} Wanajo, S., Sekiguchi, 
Y., Nishimura, N., et al.\ 2014, \apjl, 789, L39

\end{thebibliography}

